Order $p$ quantum Wasserstein distances from couplings

Optimal transport provides a powerful mathematical framework with applications spanning numerous fields. A cornerstone within this domain is the $p$-Wasserstein distance, which serves to quantify the cost of transporting one probability measure to another. While recent attempts have sought to extend this measure to the realm of quantum states, existing definitions often present certain limitations, such as not being faithful. In this work, we present a new definition of quantum Wasserstein distances. This definition, leveraging the coupling method and a metric applicable to pure states, draws inspiration from a property characterising the classical Wasserstein distance - its determination based on its value on point masses. Subject to certain continuity properties, our definition exhibits numerous attributes expected of an optimal quantum rendition of the Wasserstein distance. Notably, our approach seamlessly integrates metrics familiar to quantum information theory, such as the trace distance. Moreover, it provides an organic extension for metrics, like Nielsen's complexity metric, allowing their application to mixed states with a natural operational interpretation. Furthermore, we analyze this metric's attributes in the context of random quantum states and unveil phase transitions concerning the complexity of subsystems of random states.

==> macros.tex <==
\newcommand{\C}{{\mathbb{C}}} 
\newcommand{\R}{{\mathbb{R}}}

\newcommand{\one}{{\mathbbm{1}}} % identity matrix 

\DeclareMathOperator*{\E}{\mathbb{E}}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\spec}{Spec}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\gen}{gen} % generalisation
\DeclareMathOperator{\id}{id} % identity op
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\bigO}{\mathcal{O}}
\DeclareMathOperator{\smallO}{\mathrm{o}}
\DeclareMathOperator{\ii}{\mathrm{i}}
\DeclareMathOperator{\ee}{\mathrm{e}}

\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cH}{\mathcal{H}} % Hilbert
\newcommand{\cB}{\mathcal{B}} % bounded operators
\newcommand{\cT}{\mathcal{T}} % trace class
\newcommand{\alg}{\mathcal{A}} % the learner
\newcommand{\eps}{\epsilon}


\newcommand{\polylog}{\text{poly}\log}
\newcommand{\cc}[1]{\mathsf{{#1}}}	% complexity class

\newcommand{\Norm}[1]{\left\|{#1}\right\|}
\newcommand{\Abs}[1]{\left|{#1}\right|}
\newcommand{\Tr}[1]{\tr\left({#1}\right)}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor}
\newcommand{\ceil}[1]{\left \lceil #1 \right \rceil}


\newcommand{\ketbra}[2]{\ket{#1}\!\!\bra{#2}}
\newcommand{\proj}[1]{\ketbra{{#1}}{{#1}}}

\newcommand{\question}[1]{\textcolor{magenta}{#1}}
\newcommand{\comment}[1]{\textcolor{blue}{#1}}
\newcommand{\parahead}[1]{\noindent\textbf{{#1}}} 
\newcommand{\norm}[1]{\left\|#1\right\|}
